Bridging the Gap between Intermediate and Massive Stars I: Validation of MESA against the State-of-the-Art Monash Stellar Evolution Program for a 2$M_{\odot}$ AGB Star

One--dimensional stellar structure and evolution programs are built using different physical prescriptions and algorithms, which means there can be variations between models' predictions even when using identical input physics. This leads to questions about whether such deviations are physical or numerical; code validation studies are important and necessary tools for studying these questions. We provide the first direct comparison between the Monash stellar evolution program and MESA for a $2M_{\odot}$ model evolved from the zero-age main sequence to the tip of the thermally pulsing asymptotic giant branch. We compare the internal structure of the two models at six critical evolutionary points and find that they are in excellent agreement in characteristics like central temperature, central density and the temperature at the base of the convective envelope during the thermally pulsing asymptotic giant branch. The hydrogen-exhausted core mass between the models differs by less than 4.2% throughout the entire evolution, the final values vary only by 1.5%. Surface quantities such as luminosity and radius vary by less than 0.2% prior to the asymptotic giant branch. During thermal pulses, the difference extends to 3.4%, largely due to uncertainties in mixing and the treatment of atmospheric boundary conditions. Given that the veteran Monash code is closed source, the present work provides the first fully open-source computational analog. This increases accessibility to precision modeling on the asymptotic giant branch and lays the groundwork for higher-mass calculations that are performed with MESA but preserve the standards of the Monash code during the AGB.

==> scratch.tex <==
% \section{to-do-list}

% \begin{enumerate}
%     % \item \mj{add commentary about memory}
%     %\item  DONE \mj{\citet{Wood1981}
%     %https://ui.adsabs.harvard.edu/abs/1981ApJ...248..311W/abstract 
%     %}
%     %\item DONE \mj{Monash doesn't actually use Jina reaclib, it uses ... something 88, but particular reactions have been updated to modern values from ... easy to check this in the energy subroutine}
%     %\item DONE \mj{Peter Wood 1974 paper on thermal pulses?}
%     %https://ui.adsabs.harvard.edu/abs/1973ApJ...181..147W/abstract
%     %https://ui.adsabs.harvard.edu/abs/1974ApJ...190..609W/abstract 
    
%     \item MERIDITH \mj{How Monash treats entropy -- Peter Wood, 1981}
    
%   % \item GIULIA \mj{cite Lattanzio 91 in convection section 2.4; Semi--convection and core helium burning -- Lattanzio 1991}
%     %\item DONE \mj{Hot bottom burning -- \citet{Lattanzio1996}}
%     %\item DONE \mj{note that radius at AGB is definted at T = Teff (place where atm is patched) in Monash}
%     %\item GIULIA \mj{make clear that the reason for spikes in the HRD and in the surface quantity panels for the Monash model is a lack of convergence (these spikes are common in models produced by other AGB codes). MESA is designed to converge, so this doesn't happen to us, but MESA pays for it in run time. Numerical instabilities occur when luminosities are large. See Betelgeuse paper \citet{Joyce2020}}
%     %\item GIULIA \mj{two sentences for every figure in the appendix: (1) this is blah; (2) blah compared to its analogue in the main text is blah2}
%     %\item \mj{add MESA appendix from best practices}
% \end{enumerate}
